The Categorification of a Symmetric Operad is Independent of Signature

Given a symmetric operad $P$, and a signature (or generating sequence) $\Phi$ for $P$, we define a notion of the "categorification" (or "weakening") of $P$ with respect to $\Phi$. When $P$ is the symmetric operad whose algebras are commutative monoids, with the standard signature, we recover the notion of symmetric monoidal categories. We then show that this categorification is independent (up to equivalence) of the choice of signature.

==> dops.tex <==
% "Distributive operad" terminology, to save typing and in case I change my
% mind.
\newcommand{\dop}{distributive operad}
\newcommand{\Dop}{Distributive operad}
\newcommand{\DOp}{Distributive Operad}
\newcommand{\dm}{distributive multicategory}
\newcommand{\Dm}{Distributive multicategory}
\newcommand{\DM}{Distributive Multicategory}
\newcommand{\dops}{distributive operads}
\newcommand{\Dops}{Distributive operads}
\newcommand{\DOps}{Distributive Operads}
\newcommand{\dms}{distributive multicategories}
\newcommand{\Dms}{Distributive multicategories}
\newcommand{\DMs}{Distributive Multicategories}
\newcommand{\dco}{distributive \Cat-operad}
\newcommand{\Dco}{Distributive \Cat-operad}
\newcommand{\DCO}{Distributive \Cat-Operad}
\newcommand{\dcm}{distributive \Cat-multicategory}
\newcommand{\Dcm}{Distributive \Cat-multicategory}
\newcommand{\DCM}{Distributive \Cat-Multicategory}
\newcommand{\dcos}{distributive \Cat-operads}
\newcommand{\Dcos}{Distributive \Cat-operads}
\newcommand{\DCOs}{Distributive \Cat-Operads}
\newcommand{\dcms}{distributive \Cat-multicategories}
\newcommand{\Dcms}{Distributive \Cat-multicategories}
\newcommand{\DCMs}{Distributive \Cat-Multicategories}
\newcommand{\DOpCat}{{\rm\textbf{DOp}}}
\newcommand{\DCOCat}{{\rm\textbf{DCO}}}
\newcommand{\DOpstr}{{\rm\textbf{DOp}\ensuremath{_{\mbox{\small str}}}}}
\newcommand{\DCOstr}{{\rm\textbf{DCO}\ensuremath{_{\mbox{\small str}}}}}
\newcommand{\DOpwk}{{\rm\textbf{DOp}\ensuremath{_{\mbox{\small wk}}}}}
\newcommand{\DCOwk}{{\rm\textbf{DCO}\ensuremath{_{\mbox{\small wk}}}}}
\newcommand{\DOplax}{{\rm\textbf{DOp}\ensuremath{_{\mbox{\small lax}}}}}
\newcommand{\DCOlax}{{\rm\textbf{DCO}\ensuremath{_{\mbox{\small lax}}}}}


==> utils.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
\DeclareMathSymbol{\natural}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\integer}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\real}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\rational}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\I}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\complex}{\mathbin}{AMSb}{"43}
\DeclareMathSymbol{\bbF}{\mathbin}{AMSb}{"46}
\DeclareMathSymbol{\bbI}{\mathbin}{AMSb}{"49}
\newcommand{\C}{\ensuremath{\mathcal{C}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\F}{\ensuremath{\bbF}}
\newcommand{\defterm}[1]{\textbf{#1}}
\newcommand{\Alg}{\textbf{Alg}}
\newcommand{\Algwk}{\textbf{Alg}_{\textrm{wk}}}
\newcommand{\Cat}{\textbf{Cat}}
\newcommand{\CAT}{\textbf{CAT}}
\newcommand{\Set}{\textbf{Set}}
\newcommand{\Digraph}{\textbf{Digraph}}
\newcommand{\Operad}{\textbf{Operad}}
\newcommand{\SymmOperad}{\textbf{$\Sigma$-Operad}}
\newcommand{\CatOperad}{\textbf{Cat-Operad}}
\newcommand{\CatSymmOperad}{\textbf{Cat-$\Sigma$-Operad}}
\newcommand{\VOperad}{\textbf{$\mathcal{V}$-Operad}}
\newcommand{\VSymmOperad}{\textbf{$\mathcal{V}$-$\Sigma$-Operad}}
\newcommand{\Fill}{\mbox{\rm\textbf{Fill}}}
\newcommand{\End}{\mathop{\mbox{\rm{End}}}}
\newcommand{\dt}{.\linebreak[0]}     % used to allow linebreaks in URLs
\newcommand{\slbrk}{/\linebreak[0]}  % especially in bibliographies
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}

